Learning Quasi-Static 3D Models of Markerless Deformable Linear Objects for Bimanual Robotic Manipulation

The robotic manipulation of Deformable Linear Objects (DLOs) is a vital and challenging task that is important in many practical applications. Classical model-based approaches to this problem require an accurate model to capture how robot motions affect the deformation of the DLO. Nowadays, data-driven models offer the best tradeoff between quality and computation time. This paper analyzes several learning-based 3D models of the DLO and proposes a new one based on the Transformer architecture that achieves superior accuracy, even on the DLOs of different lengths, thanks to the proposed scaling method. Moreover, we introduce a data augmentation technique, which improves the prediction performance of almost all considered DLO data-driven models. Thanks to this technique, even a simple Multilayer Perceptron (MLP) achieves close to state-of-the-art performance while being significantly faster to evaluate. In the experiments, we compare the performance of the learning-based 3D models of the DLO on several challenging datasets quantitatively and demonstrate their applicability in the task of shaping a DLO.

==> rw_identification.tex <==
\cite{caldwell2014identification} -- 
\url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=6942666}
\begin{itemize}
    \item identification of a flexible loop based on the discrete dynamics parameters
    \item 
\end{itemize}


\cite{liu2023pbd} -- 
\url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10093017}
\begin{itemize}
    \item parameter estimation through the differnetiable model based on position based dynamics
    \item markers
    \item no rotations applied
    \item needs at least a few seconds to evaluate
    \item 
\end{itemize}


\cite{alvarez2016identification} -- 
\url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7862387}
\begin{itemize}
    \item they are simulating the cable with different parameters in some engine and trying to find out what is the best set of parameters that explains the observations 
    \item 
\end{itemize}
